Trajectory-Optimized Sensing for Active Search of Tissue Abnormalities in Robotic Surgery

In this work, we develop an approach for guiding robots to automatically localize and find the shapes of tumors and other stiff inclusions present in the anatomy. Our approach uses Gaussian processes to model the stiffness distribution and active learning to direct the palpation path of the robot. The palpation paths are chosen such that they maximize an acquisition function provided by an active learning algorithm. Our approach provides the flexibility to avoid obstacles in the robot's path, incorporate uncertainties in robot position and sensor measurements, include prior information about location of stiff inclusions while respecting the robot-kinematics. To the best of our knowledge this is the first work in literature that considers all the above conditions while localizing tumors. The proposed framework is evaluated via simulation and experimentation on three different robot platforms: 6-DoF industrial arm, da Vinci Research Kit (dVRK), and the Insertable Robotic Effector Platform (IREP). Results show that our approach can accurately estimate the locations and boundaries of the stiff inclusions while reducing exploration time.

==> CEM_ErgodicCoverage.tex <==
In this section, we introduce a formulation that optimizes an ergodic coverage objective using the stochastic trajectory optimization algorithm presented in Section~\ref{sec:CEM}. In this formulation, we pose ergodic coverage as a constrained optimization problem subject to constraints associated with obstacle avoidance and with the motion model of the robot. We start by redefining the time average statistics of a robot's trajectory to capture the robot's sensor footprint. We then demonstrate that obstacle avoidance can be easily incorporated into this framework by giving penalties to the sampled trajectories that collide with arbitrarily-shaped obstacles or that cross restricted regions.

Let us start with two key observations. First,  Eq.~(\ref{eq:time-average}) assumes that a robot's trajectory is composed of Dirac delta functions. In other words, it is assumed that the sensor  footprint is negligible compared to the size of the domain. This assumption is adopted to efficiently calculate the Fourier coefficients of the distributions given by Eq.~(\ref{eq:Fourier_coefficients}). In many practical applications, the robots can be equipped with sensors of various types  (camera, lidar, ultrasonic, etc.), which are hardly captured by the Dirac delta function. Having control over the sensor footprint opens up interesting and useful strategies for coverage:  a robot equipped with a wide sensor footprint should be able to perform a coarse ergodic coverage of the domain compared to a robot equipped with a narrow sensor footprint. Similarly, the optimal ergodic-coverage trajectory of a ground vehicle equipped with a forward looking ultrasonic sensor would be different than an aerial vehicle equipped with a downward-looking sensor.

Second, as also stated in ~\cite{miller2013},  the motivation in using the norm on the Fourier coefficients is to obtain an objective function that is differentiable with respect to the trajectory. When a sampling-based approach is used for trajectory optimization, there is no need for a differentiable objective function. There are many other measures used in information theory and statistics to compare two distributions. Here, we consider Kullback-Leibler (KL) divergence, which measures the relative entropy between two distributions,
\begin{equation}
\label{eq:KLdiv}
D_{KL}(\Gamma \vert \xi)=\int_{X}\Gamma(\bm{x}) \log\left(\frac{\Gamma(\bm{x})}{\xi(\bm{x})}\right)d\bm{x}.
\end{equation}
KL divergence can encode an ergodic coverage objective without resorting to the spectral decomposition of the desired coverage distribution, whose accuracy is limited by the number of basis functions used. Additionally, we can explicitly measure the ergodicity of a trajectory without resorting to simplifications in the representation of a robot's sensor footprint. 

In our formulation, the optimal control problem posed in Eq. (\ref{eq:CEM_cost}) can be solved by defining the cost function $J(\textbf{z})$ to be 
\begin{equation}
J(\textbf{z}) = D_{KL}(\Gamma \vert \xi)
\end{equation}
where $z$ is sampled from a Gaussian mixture model defined in Eq. (\ref{eq:GMM}).

\subsection{Obstacle Avoidance}
Suppose that the domain $X$ contains $p$ obstacles denoted by $O_1,..., O_p \subset X$. We assume that the robot at state $\bm{q}$ is occupying a region $A(\bm{q})\subset X$. Borrowing the notation in \cite{kobilarov2012cross}, let the function \textbf{prox}($A_1,A_2$) return the closest Euclidean distance between two sets $A_{1,2} \subset X$. This function returns a negative value if the two sets intersect. Therefore, for an agent to avoid the obstacles $O_1,...,O_p$, we impose a constraint of the form of Eq.~(\ref{eq:constraints}) expressed as,
\begin{equation}\label{eq:constraint}
F(\bm{q}(t)) = \min_i \mbox{\textbf{prox}}(A(\bm{q}(t)),O_i), ~ \forall t\in[0,\infty).
\end{equation}

The sampled trajectories that does not  satisfy the constraints of Eq. (\ref{eq:constraints})  are penalized.

\subsection{Example: Dubins Car}
The trajectory optimization framework can be applied to any robot whose dynamics are given as (\ref{eq:dynamics}) given that we can parameterize the space of all trajectories satisfying (\ref{eq:dynamics}) using motion primitives. We will consider the Dubins car model whose motion is restricted to a plane. The state space for such a model is $Q = SE(2)$ with state $\bm{q} = (x, y , \theta)$, where $(x, y)$ are the Cartesian coordinates of the robot, and $\theta$ is the orientation of the robot in the plane. The dynamics of a dubins car is defined by,
\begin{equation}\label{dubins}
\dot{x} = u\cos\theta ,~~~  \dot{y} = u\sin\theta,~~~   \dot{\theta} = v
\end{equation}
where $v \in [v_{min}, v_{max}]$ is a controlled forward velocity, and $w \in [w_{min}, w_{max}]$ is a controlled turning rate.

We can represent a trajectory satisfying (\ref{dubins}) as a set of connected motion primitives consisting of either straight lines with constant velocity $v$ or arcs of radius $v/w$. We define a primitive by a constant controls ($v, w$). The duration of each primitive is constant and $\tau > 0$. We parameterize the trajectory of the robot using $m$ primitives, and this finite dimensional parameterization is represented by  a vector $\bm{z} \in \mathbb{R}^{2m}$ such that,
\begin{equation}
\bm{z} = (v_1,w_1, ..., v_m, w_m) 
\end{equation}

The $j^{th}$ primitive ends at time $t_j = j\tau$ for $j \in {1,..,m}$. For any time $t \in [t_j, t_{j+1}]$, the parameterization $\varphi_z = (v, w, x, y ,\theta)$ is given by,
\begin{align}\nonumber
v(t) &= v_{j+1}
\\\nonumber
w(t) &= w_{j+1}
\\
\theta(t) &= \theta_j + w_{j+1}\Delta t_j
\\\nonumber
x(t) &= \left\{
\begin{array}{ll}
x(t_j) + \frac{v_{j+1}}{w_{j+1}}(\sin(\theta(t))-\sin\theta_j),  & \mbox{if } w_{j+1}\neq0 \\
x(t_j) + v_{j+1} \Delta t_j\cos\theta_j, &  otherwise
\end{array}
\right.
\\\nonumber
y(t) &= \left\{
\begin{array}{ll}
y(t_j) + \frac{v_{j+1}}{w_{j+1}}(\cos\theta_j - \cos(\theta(t))),  & \mbox{if } w_{j+1}\neq0 \\
y(t_j) + v_{j+1} \Delta t_j\sin\theta_j, &  otherwise
\end{array}
\right.
\end{align}
where $\theta_j = \theta(t_j)$ and $\Delta t_j = t - t_j$.

==> Results.tex <==
\subsection{Simulation Results}

\subsubsection{Discrete Probing}

\subsubsection{Continuous Probing}



\subsection{Experimental Results}

\subsubsection{Foxbot Robot}
\subsubsection{Da Vinci Research Kit}
\subsubsection{IREP}

